Low-memory GEMM-based convolution algorithms for deep neural networks

Deep neural networks (DNNs) require very large amounts of computation both for training and for inference when deployed in the field. A common approach to implementing DNNs is to recast the most computationally expensive operations as general matrix multiplication (GEMM). However, as we demonstrate in this paper, there are a great many different ways to express DNN convolution operations using GEMM. Although different approaches all perform the same number of operations, the size of temporary data structures differs significantly. Convolution of an input matrix with dimensions $C \times H \times W$, requires $O(K^2CHW)$ additional space using the classical im2col approach. More recently memory-efficient approaches requiring just $O(KCHW)$ auxiliary space have been proposed. We present two novel GEMM-based algorithms that require just $O(MHW)$ and $O(KW)$ additional space respectively, where $M$ is the number of channels in the result of the convolution. These algorithms dramatically reduce the space overhead of DNN convolution, making it much more suitable for memory-limited embedded systems. Experimental evaluation shows that our low-memory algorithms are just as fast as the best patch-building approaches despite requiring just a fraction of the amount of additional memory. Our low-memory algorithms have excellent data locality which gives them a further edge over patch-building algorithms when multiple cores are used. As a result, our low memory algorithms often outperform the best patch-building algorithms using multiple threads.

==> pbqp.tex <==
\section{Selecting the best primitives}
\label{sec:pbqp}

A deep neural network consists of a directed graph of \textit{layers}
that receive, process and output data. In the best known DNNs, such as
convolutional NNs, the network is a directed acyclic graph of
layers. We concentrate primarily on acyclic DNNs.

Data flows between \textit{layers} along directed edges. A DNN can be
implemented using a library of \textit{primitive} routines. Each
primitive implements a standard DNN operator such as convolution,
activation, a fully-connected layer, and so forth. In addition, a
primitive might perform a sequence of DNN layers: for example, a
single primitive might perform an activation function, such as ReLU,
convolution on the result, followed by another activation. Primitives
may be programmed manually, or generated by a domain-specific code
generator for DNNs.

Each primitive takes inputs in a given data layout, performs the
operations of one or more layers, and produces output in a given
format. Some DNN libraries produce all inputs and outputs in a
canonical form, such as $NCHW$ used by Caffe
\cite{is-this-correct?}. However, forcing each layer to use the same
format arguably removes the opportunity to customize layouts to
particular operations (such as convolution with large $K$ but small
$C$) or for cross-layer optimizations that exploit particular layouts.

A simple way to find the cost of implementing any layer with any
primitive is to execute the primitive using sample inputs for the
layer. The control flow of execution of most DNN layers depends
primarily on the dimensions of the input rather than on the input
values. The execution time tends to remain stable regardless of the
particular input values, and it is therefore possible to measure with
some consistency the execution time of a given primitive implementing
a given layer. However, given a set of execution times for
implementing the various layers with different primitives, it is not
obvious which primitives to select for which layers.

% In particular, when input data is converted
% to a special format, such as the Fourier domain, it may be more
% efficient to keep the data in Fourier format rather than to convert
% back and forth on each layer.

\subsection{The Problem}
In this section we consider the problem of selecting the lowest cost
set of primitives to implement a DNN. By lowest cost we mean that the
sum of the execution time of each of the primitives that implement
the DNN is minimized. This problem may seem no more than selecting
the fastest implementation of each layer, but in fact it is more
difficult for two reasons:
\begin{itemize}
\item A single primitive function may implement more than one node (layer)
  of the graph, which raises the problem of selecting between different
  overlapping matchings of a group of nodes.
\item Each primitive function deals with inputs and outputs in a
  particular data format. If the output data format of one primitive
  does not match the input data format of a direct successor, then a
  data format conversion must be inserted between the two if they are
  to be selected. The cost of the data conversions increases the total
  cost of the selection.
\end{itemize}

\noindent The first of these is similar to the problem of a compiler
selecting machine instructions to implement and expression graph.
Instruction selection on DAGs is known to be NP-hard \cite{}. In the
next section we propose a solution to both problems within a single
framework.

\subsection{Our solution}
The partitioned Boolean quadratic programming (PBQP) problem \cite{}
is a specific type of assignment problem. Given a set of layers and a
set of primitives, we attempt to assign the layers to primitives to
minimize the total cost. The cost of assigning a layer to a primitive
is the execution time of the layer implemented with that primitive.

Figure \ref{} shows a simple graph representation of a PBQP instance.
Each layer can be implemented by any one of four different primitives.
Each of the primitives uses a different algorithm, and therefore has
a different cost to implement the layer.


In addition to the layer costs, a second set of costs can be
associated with the edges of the graph. These edge costs capture
additional costs that arise from the \textit{pair of selections} made
at each end of the edge. Each of our primitives accepts input in a
particular data format and produces output in a format (which is
often, but not always, the same as the input format). If the output
format of a producer primitive does not match the input format
of a consumer 


Figure \ref{} shows a $4 \times4$ 2D table on
the edge, which represents the cost of transitioning between on


the cost
%
% Our proposed solution models the primitive selection problem as a
% partitioned Boolean quadratic programming (PBQP) problem \cite{}.
% PBQP has been used extensively in compiler optimization for problems
% such as instruction selection and register allocation. Figure \ref{}
% shows an example of covering a DNN graph with primitive routines.  In
% this example, we assume that each primitive implements exactly one DNN
% layer at a given cost in execution time. Alongside each layer of the
% DNN graph is a small 1D table showing the cost of selecting any one of
% the primitives to implement that layer.

In addition to the cost table for each individual layer, the PBQP
formulation allows a second cost to be specified for edges.
In our simple example, a cost table is associated with each edge in
the graph as well as each node. This is a 2D cost table that
represents the costs associated with pairs of selections on each of
the nodes connected by the edge. For example, in Figure \ref{}
primitive \texttt{conv\_hwc} is the lowest cost match for layer
\texttt{Conv3x3} and \texttt{relu\_chw} is for layer \texttt{ReLU}.
However, there is also a cost arising from this combination of
primitives on the edge between the two layers. In the example, the
edge cost is large because the two primitives use different data
layouts, and therefore a data layout transformation must be inserted
between the two primitives. The additional cost that arises from pairs
of assignment choices on the graph edges makes PBQP different from
other similar problems, such as the \textit{assignment problem}
\cite{Munkres57}.

Data format transformation costs on graph edges are particularly
problematic in DAG-shaped DNNs. Where a layer has multiple direct
successors and/or predecessors, the same data format may not be
optimal for all. Choosing one format over another may limit the choice
of primitives that can be used in successor/predecessor layers, or may
require the insertion of expensive data format transformations.
PBQP allows us to model these dependent costs within an abstract
optimization problem.

\subsection{Our problem formulation}
In addition to modelling data formats and transformation costs, we
also model the selection of \textit{fused primitives} in PBQP.  A
fused primitive is one that matches more than one layer in the DNN
graph. For example, in many DNNs convolution layers are normally
followed by an activation layer, such as ReLU. Many DNN libraries
provide a fused \texttt{Conv-ReLU} primitive that performs both
operations. More complicated fused primitives are also possible, such
longer sequences of layers, and tree- or DAG-shaped groups of layers.

Figure \ref{} shows an example of a set of primitives that can
match more than one DNN layer, such as a primitive that
can match a \texttt{Conv3x3} layer followed by a \texttt{ReLU}
layer. 


